Measurement of $e^{+}e^{-} \to K^{+}K^{-}\pi^{0}$ cross section and observation of a resonant structure

Based on $e^{+}e^{-}$ collision data collected by the BESIII detector at the BEPCII collider at center-of-mass energies from 2.000 to 3.080 GeV, a partial-wave analysis is performed for the process $e^{+}e^{-} \to K^{+}K^{-}\pi^{0}$. The Born cross section of the process $e^{+}e^{-} \to K^{+}K^{-}\pi^{0}$ and its subprocesses $e^{+}e^{-} \to \phi \pi^{0}$, $K^{*}(892)K$ and $K^{*}_{2}(1430)K$ are measured. The results for $e^{+}e^{-} \to K^{+}K^{-}\pi^{0}$ and $\phi \pi^{0}$ are consistent with the BaBar measurements and with improved precision. By analyzing the cross section, of the subprocesses $e^{+}e^{-} \to$ $K^{*}(892)K$ and $K^{*}_{2}(1430)K$, a structure with mass $M_R$ = (2208 $\pm$ 19 $\pm$ 24) MeV/$c^{2}$ and width $\Gamma_R$ = (168 $\pm$ 24 $\pm$ 39) MeV is observed with a combined statistical significance of 7.6$\sigma$. The measured resonance parameters suggest it can be identified as the $\phi(2170)$, thus the results provide valuable input to understand the internal nature of this state.

==> authorv1.tex <==
%\author{Author list}
%\begin{small}
%\begin{center}
\noindent
M.~Ablikim$^{1}$, M.~N.~Achasov$^{10,b}$, P.~Adlarson$^{67}$, S. ~Ahmed$^{15}$, M.~Albrecht$^{4}$, R.~Aliberti$^{28}$, A.~Amoroso$^{66A,66C}$, M.~R.~An$^{32}$, Q.~An$^{63,49}$, X.~H.~Bai$^{57}$, Y.~Bai$^{48}$, O.~Bakina$^{29}$, R.~Baldini Ferroli$^{23A}$, I.~Balossino$^{24A}$, Y.~Ban$^{38,i}$, K.~Begzsuren$^{26}$, N.~Berger$^{28}$, M.~Bertani$^{23A}$, D.~Bettoni$^{24A}$, F.~Bianchi$^{66A,66C}$, J.~Bloms$^{60}$, A.~Bortone$^{66A,66C}$, I.~Boyko$^{29}$, R.~A.~Briere$^{5}$, H.~Cai$^{68}$, X.~Cai$^{1,49}$, A.~Calcaterra$^{23A}$, G.~F.~Cao$^{1,54}$, N.~Cao$^{1,54}$, S.~A.~Cetin$^{53A}$, J.~F.~Chang$^{1,49}$, W.~L.~Chang$^{1,54}$, G.~Chelkov$^{29,a}$, D.~Y.~Chen$^{6}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,54}$, M.~L.~Chen$^{1,49}$, S.~J.~Chen$^{35}$, X.~R.~Chen$^{25}$, Y.~B.~Chen$^{1,49}$, Z.~J~Chen$^{20,j}$, W.~S.~Cheng$^{66C}$, G.~Cibinetto$^{24A}$, F.~Cossio$^{66C}$, X.~F.~Cui$^{36}$, H.~L.~Dai$^{1,49}$, X.~C.~Dai$^{1,54}$, A.~Dbeyssi$^{15}$, R.~ E.~de Boer$^{4}$, D.~Dedovich$^{29}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{28}$, I.~Denysenko$^{29}$, M.~Destefanis$^{66A,66C}$, F.~De~Mori$^{66A,66C}$, Y.~Ding$^{33}$, C.~Dong$^{36}$, J.~Dong$^{1,49}$, L.~Y.~Dong$^{1,54}$, M.~Y.~Dong$^{1,49,54}$, X.~Dong$^{68}$, S.~X.~Du$^{71}$, Y.~L.~Fan$^{68}$, J.~Fang$^{1,49}$, S.~S.~Fang$^{1,54}$, Y.~Fang$^{1}$, R.~Farinelli$^{24A}$, L.~Fava$^{66B,66C}$, F.~Feldbauer$^{4}$, G.~Felici$^{23A}$, C.~Q.~Feng$^{63,49}$, J.~H.~Feng$^{50}$, M.~Fritsch$^{4}$, C.~D.~Fu$^{1}$, Y.~Gao$^{64}$, Y.~Gao$^{63,49}$, Y.~Gao$^{38,i}$, Y.~G.~Gao$^{6}$, I.~Garzia$^{24A,24B}$, P.~T.~Ge$^{68}$, C.~Geng$^{50}$, E.~M.~Gersabeck$^{58}$, A~Gilman$^{61}$, K.~Goetzen$^{11}$, L.~Gong$^{33}$, W.~X.~Gong$^{1,49}$, W.~Gradl$^{28}$, M.~Greco$^{66A,66C}$, L.~M.~Gu$^{35}$, M.~H.~Gu$^{1,49}$, S.~Gu$^{2}$, Y.~T.~Gu$^{13}$, C.~Y~Guan$^{1,54}$, A.~Q.~Guo$^{22}$, L.~B.~Guo$^{34}$, R.~P.~Guo$^{40}$, Y.~P.~Guo$^{9,g}$, A.~Guskov$^{29,a}$, T.~T.~Han$^{41}$, W.~Y.~Han$^{32}$, X.~Q.~Hao$^{16}$, F.~A.~Harris$^{56}$, K.~L.~He$^{1,54}$, F.~H.~Heinsius$^{4}$, C.~H.~Heinz$^{28}$, T.~Held$^{4}$, Y.~K.~Heng$^{1,49,54}$, C.~Herold$^{51}$, M.~Himmelreich$^{11,e}$, T.~Holtmann$^{4}$, G.~Y.~Hou$^{1,54}$, Y.~R.~Hou$^{54}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,54}$, J.~F.~Hu$^{47,k}$, T.~Hu$^{1,49,54}$, Y.~Hu$^{1}$, G.~S.~Huang$^{63,49}$, L.~Q.~Huang$^{64}$, X.~T.~Huang$^{41}$, Y.~P.~Huang$^{1}$, Z.~Huang$^{38,i}$, T.~Hussain$^{65}$, N~H\"usken$^{22,28}$, W.~Ikegami Andersson$^{67}$, W.~Imoehl$^{22}$, M.~Irshad$^{63,49}$, S.~Jaeger$^{4}$, S.~Janchiv$^{26}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{16}$, X.~B.~Ji$^{1,54}$, X.~L.~Ji$^{1,49}$, Y.~Y.~Ji$^{41}$, H.~B.~Jiang$^{41}$, X.~S.~Jiang$^{1,49,54}$, J.~B.~Jiao$^{41}$, Z.~Jiao$^{18}$, S.~Jin$^{35}$, Y.~Jin$^{57}$, M.~Q.~Jing$^{1,54}$, T.~Johansson$^{67}$, N.~Kalantar-Nayestanaki$^{55}$, X.~S.~Kang$^{33}$, R.~Kappert$^{55}$, M.~Kavatsyuk$^{55}$, B.~C.~Ke$^{43,1}$, I.~K.~Keshk$^{4}$, A.~Khoukaz$^{60}$, P. ~Kiese$^{28}$, R.~Kiuchi$^{1}$, R.~Kliemt$^{11}$, L.~Koch$^{30}$, O.~B.~Kolcu$^{53A,d}$, B.~Kopf$^{4}$, M.~Kuemmel$^{4}$, M.~Kuessner$^{4}$, A.~Kupsc$^{67}$, M.~ G.~Kurth$^{1,54}$, W.~K\"uhn$^{30}$, J.~J.~Lane$^{58}$, J.~S.~Lange$^{30}$, P. ~Larin$^{15}$, A.~Lavania$^{21}$, L.~Lavezzi$^{66A,66C}$, Z.~H.~Lei$^{63,49}$, H.~Leithoff$^{28}$, M.~Lellmann$^{28}$, T.~Lenz$^{28}$, C.~Li$^{39}$, C.~H.~Li$^{32}$, Cheng~Li$^{63,49}$, D.~M.~Li$^{71}$, F.~Li$^{1,49}$, G.~Li$^{1}$, H.~Li$^{63,49}$, H.~Li$^{43}$, H.~B.~Li$^{1,54}$, H.~J.~Li$^{16}$, J.~L.~Li$^{41}$, J.~Q.~Li$^{4}$, J.~S.~Li$^{50}$, Ke~Li$^{1}$, L.~K.~Li$^{1}$, Lei~Li$^{3}$, P.~R.~Li$^{31,l,m}$, S.~Y.~Li$^{52}$, W.~D.~Li$^{1,54}$, W.~G.~Li$^{1}$, X.~H.~Li$^{63,49}$, X.~L.~Li$^{41}$, Xiaoyu~Li$^{1,54}$, Z.~Y.~Li$^{50}$, H.~Liang$^{63,49}$, H.~Liang$^{1,54}$, H.~~Liang$^{27}$, Y.~F.~Liang$^{45}$, Y.~T.~Liang$^{25}$, G.~R.~Liao$^{12}$, L.~Z.~Liao$^{1,54}$, J.~Libby$^{21}$, C.~X.~Lin$^{50}$, B.~J.~Liu$^{1}$, C.~X.~Liu$^{1}$, D.~~Liu$^{15,63}$, F.~H.~Liu$^{44}$, Fang~Liu$^{1}$, Feng~Liu$^{6}$, H.~B.~Liu$^{13}$, H.~M.~Liu$^{1,54}$, Huanhuan~Liu$^{1}$, Huihui~Liu$^{17}$, J.~B.~Liu$^{63,49}$, J.~L.~Liu$^{64}$, J.~Y.~Liu$^{1,54}$, K.~Liu$^{1}$, K.~Y.~Liu$^{33}$, L.~Liu$^{63,49}$, M.~H.~Liu$^{9,g}$, P.~L.~Liu$^{1}$, Q.~Liu$^{68}$, Q.~Liu$^{54}$, S.~B.~Liu$^{63,49}$, Shuai~Liu$^{46}$, T.~Liu$^{1,54}$, W.~M.~Liu$^{63,49}$, X.~Liu$^{31,l,m}$, Y.~Liu$^{31,l,m}$, Y.~B.~Liu$^{36}$, Z.~A.~Liu$^{1,49,54}$, Z.~Q.~Liu$^{41}$, X.~C.~Lou$^{1,49,54}$, F.~X.~Lu$^{50}$, H.~J.~Lu$^{18}$, J.~D.~Lu$^{1,54}$, J.~G.~Lu$^{1,49}$, X.~L.~Lu$^{1}$, Y.~Lu$^{1}$, Y.~P.~Lu$^{1,49}$, C.~L.~Luo$^{34}$, M.~X.~Luo$^{70}$, P.~W.~Luo$^{50}$, T.~Luo$^{9,g}$, X.~L.~Luo$^{1,49}$, X.~R.~Lyu$^{54}$, F.~C.~Ma$^{33}$, H.~L.~Ma$^{1}$, L.~L. ~Ma$^{41}$, M.~M.~Ma$^{1,54}$, Q.~M.~Ma$^{1}$, R.~Q.~Ma$^{1,54}$, R.~T.~Ma$^{54}$, X.~X.~Ma$^{1,54}$, X.~Y.~Ma$^{1,49}$, F.~E.~Maas$^{15}$, M.~Maggiora$^{66A,66C}$, S.~Maldaner$^{4}$, S.~Malde$^{61}$, Q.~A.~Malik$^{65}$, A.~Mangoni$^{23B}$, Y.~J.~Mao$^{38,i}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{66A,66C}$, Z.~X.~Meng$^{57}$, J.~G.~Messchendorp$^{55}$, G.~Mezzadri$^{24A}$, T.~J.~Min$^{35}$, R.~E.~Mitchell$^{22}$, X.~H.~Mo$^{1,49,54}$, Y.~J.~Mo$^{6}$, N.~Yu.~Muchnoi$^{10,b}$, H.~Muramatsu$^{59}$, S.~Nakhoul$^{11,e}$, Y.~Nefedov$^{29}$, F.~Nerling$^{11,e}$, I.~B.~Nikolaev$^{10,b}$, Z.~Ning$^{1,49}$, S.~Nisar$^{8,h}$, S.~L.~Olsen$^{54}$, Q.~Ouyang$^{1,49,54}$, S.~Pacetti$^{23B,23C}$, X.~Pan$^{9,g}$, Y.~Pan$^{58}$, A.~Pathak$^{1}$, A.~~Pathak$^{27}$, P.~Patteri$^{23A}$, M.~Pelizaeus$^{4}$, H.~P.~Peng$^{63,49}$, K.~Peters$^{11,e}$, J.~Pettersson$^{67}$, J.~L.~Ping$^{34}$, R.~G.~Ping$^{1,54}$, S.~Pogodin$^{29}$, R.~Poling$^{59}$, V.~Prasad$^{63,49}$, H.~Qi$^{63,49}$, H.~R.~Qi$^{52}$, K.~H.~Qi$^{25}$, M.~Qi$^{35}$, T.~Y.~Qi$^{9}$, S.~Qian$^{1,49}$, W.~B.~Qian$^{54}$, Z.~Qian$^{50}$, C.~F.~Qiao$^{54}$, L.~Q.~Qin$^{12}$, X.~P.~Qin$^{9}$, X.~S.~Qin$^{41}$, Z.~H.~Qin$^{1,49}$, J.~F.~Qiu$^{1}$, S.~Q.~Qu$^{36}$, K.~H.~Rashid$^{65}$, K.~Ravindran$^{21}$, C.~F.~Redmer$^{28}$, A.~Rivetti$^{66C}$, V.~Rodin$^{55}$, M.~Rolo$^{66C}$, G.~Rong$^{1,54}$, Ch.~Rosner$^{15}$, M.~Rump$^{60}$, H.~S.~Sang$^{63}$, A.~Sarantsev$^{29,c}$, Y.~Schelhaas$^{28}$, C.~Schnier$^{4}$, K.~Schoenning$^{67}$, M.~Scodeggio$^{24A,24B}$, D.~C.~Shan$^{46}$, W.~Shan$^{19}$, X.~Y.~Shan$^{63,49}$, J.~F.~Shangguan$^{46}$, M.~Shao$^{63,49}$, C.~P.~Shen$^{9}$, H.~F.~Shen$^{1,54}$, P.~X.~Shen$^{36}$, X.~Y.~Shen$^{1,54}$, H.~C.~Shi$^{63,49}$, R.~S.~Shi$^{1,54}$, X.~Shi$^{1,49}$, X.~D~Shi$^{63,49}$, J.~J.~Song$^{41}$, W.~M.~Song$^{27,1}$, Y.~X.~Song$^{38,i}$, S.~Sosio$^{66A,66C}$, S.~Spataro$^{66A,66C}$, K.~X.~Su$^{68}$, P.~P.~Su$^{46}$, F.~F. ~Sui$^{41}$, G.~X.~Sun$^{1}$, H.~K.~Sun$^{1}$, J.~F.~Sun$^{16}$, L.~Sun$^{68}$, S.~S.~Sun$^{1,54}$, T.~Sun$^{1,54}$, W.~Y.~Sun$^{27}$, W.~Y.~Sun$^{34}$, X~Sun$^{20,j}$, Y.~J.~Sun$^{63,49}$, Y.~K.~Sun$^{63,49}$, Y.~Z.~Sun$^{1}$, Z.~T.~Sun$^{1}$, Y.~H.~Tan$^{68}$, Y.~X.~Tan$^{63,49}$, C.~J.~Tang$^{45}$, G.~Y.~Tang$^{1}$, J.~Tang$^{50}$, J.~X.~Teng$^{63,49}$, V.~Thoren$^{67}$, W.~H.~Tian$^{43}$, Y.~T.~Tian$^{25}$, I.~Uman$^{53B}$, B.~Wang$^{1}$, C.~W.~Wang$^{35}$, D.~Y.~Wang$^{38,i}$, H.~J.~Wang$^{31,l,m}$, H.~P.~Wang$^{1,54}$, K.~Wang$^{1,49}$, L.~L.~Wang$^{1}$, M.~Wang$^{41}$, M.~Z.~Wang$^{38,i}$, Meng~Wang$^{1,54}$, W.~Wang$^{50}$, W.~H.~Wang$^{68}$, W.~P.~Wang$^{63,49}$, X.~Wang$^{38,i}$, X.~F.~Wang$^{31,l,m}$, X.~L.~Wang$^{9,g}$, Y.~Wang$^{63,49}$, Y.~Wang$^{50}$, Y.~D.~Wang$^{37}$, Y.~F.~Wang$^{1,49,54}$, Y.~Q.~Wang$^{1}$, Y.~Y.~Wang$^{31,l,m}$, Z.~Wang$^{1,49}$, Z.~Y.~Wang$^{1}$, Ziyi~Wang$^{54}$, Zongyuan~Wang$^{1,54}$, D.~H.~Wei$^{12}$, F.~Weidner$^{60}$, S.~P.~Wen$^{1}$, D.~J.~White$^{58}$, U.~Wiedner$^{4}$, G.~Wilkinson$^{61}$, M.~Wolke$^{67}$, L.~Wollenberg$^{4}$, J.~F.~Wu$^{1,54}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{1,54}$, X.~Wu$^{9,g}$, Z.~Wu$^{1,49}$, L.~Xia$^{63,49}$, H.~Xiao$^{9,g}$, S.~Y.~Xiao$^{1}$, Z.~J.~Xiao$^{34}$, X.~H.~Xie$^{38,i}$, Y.~G.~Xie$^{1,49}$, Y.~H.~Xie$^{6}$, T.~Y.~Xing$^{1,54}$, G.~F.~Xu$^{1}$, Q.~J.~Xu$^{14}$, W.~Xu$^{1,54}$, X.~P.~Xu$^{46}$, Y.~C.~Xu$^{54}$, F.~Yan$^{9,g}$, L.~Yan$^{9,g}$, W.~B.~Yan$^{63,49}$, W.~C.~Yan$^{71}$, Xu~Yan$^{46}$, H.~J.~Yang$^{42,f}$, H.~X.~Yang$^{1}$, L.~Yang$^{43}$, S.~L.~Yang$^{54}$, Y.~X.~Yang$^{12}$, Yifan~Yang$^{1,54}$, Zhi~Yang$^{25}$, M.~Ye$^{1,49}$, M.~H.~Ye$^{7}$, J.~H.~Yin$^{1}$, Z.~Y.~You$^{50}$, B.~X.~Yu$^{1,49,54}$, C.~X.~Yu$^{36}$, G.~Yu$^{1,54}$, J.~S.~Yu$^{20,j}$, T.~Yu$^{64}$, C.~Z.~Yuan$^{1,54}$, L.~Yuan$^{2}$, X.~Q.~Yuan$^{38,i}$, Y.~Yuan$^{1}$, Z.~Y.~Yuan$^{50}$, C.~X.~Yue$^{32}$, A.~A.~Zafar$^{65}$, X.~Zeng~Zeng$^{6}$, Y.~Zeng$^{20,j}$, A.~Q.~Zhang$^{1}$, B.~X.~Zhang$^{1}$, Guangyi~Zhang$^{16}$, H.~Zhang$^{63}$, H.~H.~Zhang$^{50}$, H.~H.~Zhang$^{27}$, H.~Y.~Zhang$^{1,49}$, J.~J.~Zhang$^{43}$, J.~L.~Zhang$^{69}$, J.~Q.~Zhang$^{34}$, J.~W.~Zhang$^{1,49,54}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,54}$, Jianyu~Zhang$^{1,54}$, Jiawei~Zhang$^{1,54}$, L.~M.~Zhang$^{52}$, L.~Q.~Zhang$^{50}$, Lei~Zhang$^{35}$, S.~Zhang$^{50}$, S.~F.~Zhang$^{35}$, Shulei~Zhang$^{20,j}$, X.~D.~Zhang$^{37}$, X.~Y.~Zhang$^{41}$, Y.~Zhang$^{61}$, Y. ~T.~Zhang$^{71}$, Y.~H.~Zhang$^{1,49}$, Yan~Zhang$^{63,49}$, Yao~Zhang$^{1}$, Z.~H.~Zhang$^{6}$, Z.~Y.~Zhang$^{68}$, G.~Zhao$^{1}$, J.~Zhao$^{32}$, J.~Y.~Zhao$^{1,54}$, J.~Z.~Zhao$^{1,49}$, Lei~Zhao$^{63,49}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{36}$, Q.~Zhao$^{1}$, S.~J.~Zhao$^{71}$, Y.~B.~Zhao$^{1,49}$, Y.~X.~Zhao$^{25}$, Z.~G.~Zhao$^{63,49}$, A.~Zhemchugov$^{29,a}$, B.~Zheng$^{64}$, J.~P.~Zheng$^{1,49}$, Y.~Zheng$^{38,i}$, Y.~H.~Zheng$^{54}$, B.~Zhong$^{34}$, C.~Zhong$^{64}$, L.~P.~Zhou$^{1,54}$, Q.~Zhou$^{1,54}$, X.~Zhou$^{68}$, X.~K.~Zhou$^{54}$, X.~R.~Zhou$^{63,49}$, X.~Y.~Zhou$^{32}$, A.~N.~Zhu$^{1,54}$, J.~Zhu$^{36}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,49,54}$, S.~H.~Zhu$^{62}$, T.~J.~Zhu$^{69}$, W.~J.~Zhu$^{36}$, W.~J.~Zhu$^{9,g}$, Y.~C.~Zhu$^{63,49}$, Z.~A.~Zhu$^{1,54}$, B.~S.~Zou$^{1}$, J.~H.~Zou$^{1}$\\
%\vspace{0.2cm}
%(BESIII Collaboration)\\

\vspace{0.2cm} {\it
\noindent
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Beijing Institute of Petrochemical Technology, Beijing 102617, People's Republic of China\\
$^{4}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{8}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{9}$ Fudan University, Shanghai 200443, People's Republic of China\\
$^{10}$ G.I. Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{11}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{12}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{13}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{14}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{15}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{16}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{17}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{18}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{19}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{20}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{21}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{22}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{23}$ INFN Laboratori Nazionali di Frascati , (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{24}$ INFN Sezione di Ferrara, (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
$^{25}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{26}$ Institute of Physics and Technology, Peace Ave. 54B, Ulaanbaatar 13330, Mongolia\\
$^{27}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{28}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{29}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{30}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{31}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{32}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{33}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{34}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{35}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{36}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{37}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{38}$ Peking University, Beijing 100871, People's Republic of China\\
$^{39}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{40}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{41}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{42}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{43}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{44}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{45}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{46}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{47}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{48}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{49}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{50}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{51}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{52}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{53}$ Turkish Accelerator Center Particle Factory Group, (A)Istanbul Bilgi University, HEP Res. Cent., 34060 Eyup, Istanbul, Turkey; (B)Near East University, Nicosia, North Cyprus, Mersin 10, Turkey\\
$^{54}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{55}$ University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{56}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{57}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{58}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{59}$ University of Minnesota, Minneapolis, Minnesota 55455, USA\\
$^{60}$ University of Muenster, Wilhelm-Klemm-Str. 9, 48149 Muenster, Germany\\
$^{61}$ University of Oxford, Keble Rd, Oxford, UK OX13RH\\
$^{62}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{63}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{64}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{65}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{66}$ University of Turin and INFN, (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{67}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{68}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{69}$ Xinyang Normal University, Xinyang 464000, People's Republic of China\\
$^{70}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{71}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
%\vspace{0.2cm}
$^{a}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{b}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{c}$ Also at the NRC ``Kurchatov Institute'', PNPI, 188300, Gatchina, Russia\\
$^{d}$ Currently at Istanbul Arel University, 34295 Istanbul, Turkey\\
$^{e}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{f}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{g}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{h}$ Also at Harvard University, Department of Physics, Cambridge, MA, 02138, USA\\
$^{i}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{j}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{k}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{l}$ Also at Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{m}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
}
%\end{center}

%\vspace{0.4cm}
%\end{small}

